Conceptualizing Machine Learning for Dynamic Information Retrieval of Electronic Health Record Notes

The large amount of time clinicians spend sifting through patient notes and documenting in electronic health records (EHRs) is a leading cause of clinician burnout. By proactively and dynamically retrieving relevant notes during the documentation process, we can reduce the effort required to find relevant patient history. In this work, we conceptualize the use of EHR audit logs for machine learning as a source of supervision of note relevance in a specific clinical context, at a particular point in time. Our evaluation focuses on the dynamic retrieval in the emergency department, a high acuity setting with unique patterns of information retrieval and note writing. We show that our methods can achieve an AUC of 0.963 for predicting which notes will be read in an individual note writing session. We additionally conduct a user study with several clinicians and find that our framework can help clinicians retrieve relevant information more efficiently. Demonstrating that our framework and methods can perform well in this demanding setting is a promising proof of concept that they will translate to other clinical settings and data modalities (e.g., labs, medications, imaging).

==> features-metadata.tex <==
\begin{table}[t]
    \centering 
    \caption{The complete list of features used in the machine learning model}
    \begin{tabular}{ll}\toprule
     Feature & Description\\\midrule
     Relative time & Difference between source note write time and target note write time\\
     Recency & How recent the target note is out of all available notes for a session\\   
     Read repetition & How many times the note in the current session was read previously \\
     Service & Clinical service of the target note (oncology, cardiology, etc.)\\
     Note type & Target note type (progress note, initial note, telephone, letter, etc.) \\ 
     Target note text & Text of entire target note\\
     \bottomrule
    \end{tabular}
  \label{tab:features_target} 
\end{table}

==> features-patient.tex <==
\begin{table}[t]
    \centering 
    \caption{Features that encode information from the source note and patient context.}
    \begin{tabular}{ll}\toprule
     Feature & Description\\\midrule
     Chief complaint & Chief complaint(s) for a patient's ED visit\\
     User information & Level of training (student, resident, attending) of the write user \\ 
     Source note text & Text of note version currently being written\\\bottomrule
    \end{tabular}
  \label{tab:features_source} 
\end{table}
